On Data Sampling Strategies for Training Neural Network Speech Separation Models

Speech separation remains an important area of multi-speaker signal processing. Deep neural network (DNN) models have attained the best performance on many speech separation benchmarks. Some of these models can take significant time to train and have high memory requirements. Previous work has proposed shortening training examples to address these issues but the impact of this on model performance is not yet well understood. In this work, the impact of applying these training signal length (TSL) limits is analysed for two speech separation models: SepFormer, a transformer model, and Conv-TasNet, a convolutional model. The WJS0-2Mix, WHAMR and Libri2Mix datasets are analysed in terms of signal length distribution and its impact on training efficiency. It is demonstrated that, for specific distributions, applying specific TSL limits results in better performance. This is shown to be mainly due to randomly sampling the start index of the waveforms resulting in more unique examples for training. A SepFormer model trained using a TSL limit of 4.42s and dynamic mixing (DM) is shown to match the best-performing SepFormer model trained with DM and unlimited signal lengths. Furthermore, the 4.42s TSL limit results in a 44% reduction in training time with WHAMR.

==> README <==

January 11, 2007


IEEEtran.bst is the official BibTeX style for authors of the Institute of
Electrical and Electronics Engineers (IEEE) Transactions journals and
conferences.

It also may have applications for other academic work such as theses and
technical reports. The alphanumeric and natbib variants extend the
applicability of the IEEEtran bibstyle family to the natural sciences
and beyond.

The IEEEtran bibstyle is a very comprehensive BibTeX style which provides
many features beyond the standard BibTeX styles, including full support
for references of online documents, patents, periodicals and standards.
See the provided user manual for detailed usage information.

The latest version of the IEEEtran BibTeX style can be found at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/bibtex/

as well as within IEEE's site:

http://www.ieee.org/

Note that the packages at IEEE's site do not contain the natbib and
alphanumeric variants (e.g., IEEEtranN.bst, etc.) as these are not used
for IEEE related work. These files can be obtained on CTAN.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtran home page at my website:

http://www.michaelshell.org/tex/ieeetran/


Enjoy!

Michael Shell
http://www.michaelshell.org/

*******
Version 1.12 (2007/01/11) changes:

 1. Fixed bug with unwanted comma before "et al." when an entry contained
    more than two author names. Thanks to Pallav Gupta for reporting this.

 2. Fixed bug with anomalous closing quote in tech reports that have a
    type, but without a number or address. Thanks to Mehrdad Mirreza for
    reporting this.

 3. Use braces in \providecommand in begin.bib to better support
    latex2html. TeX style length assignments OK with recent versions
    of latex2html - 1.71 (2002/2/1) or later is strongly recommended.
    Use of the language field still causes trouble with latex2html.
    Thanks to Federico Beffa for reporting this.

 4. Added IEEEtran.bst ID and version comment string to .bbl output.

 5. Provide a \BIBdecl hook that allows the user to execute commands
    just prior to the first entry.

 6. Use default urlstyle (is using url.sty) of "same" rather than rm to
    better work with a wider variety of bibliography styles.

 7. Changed month abbreviations from Sept., July and June to Sep., Jul.,
    and Jun., respectively, as IEEE now does. Thanks to Moritz Borgmann
    for reporting this.

 8. Control entry types should not be considered when calculating longest
    label width.

 9. Added alias www for electronic/online.

10. Updated full and abbreviated journal name string definitions in
    IEEEfull.bib and IEEEabrv.bib.

11. New IEEEtranSA.bst, IEEEtranN.bst, and IEEEtranSN.bst variants for
    alphanumeric citation tags and natbib compatibility.


********************************** Files **********************************

README                 - This file.

IEEEtran_bst_HOWTO.pdf - The user manual.

IEEEtran.bst           - The standard IEEEtran BibTeX style file. For use
                         with IEEE work.

IEEEtranS.bst          - A version of IEEEtran.bst that sorts the entries.
                         Some IEEE conferences/publications may use/allow
                         sorted bibliographies.

IEEEexample.bib        - An example BibTeX database that contains the
                         references shown in the user manual.

IEEEabrv.bib           - String definitions for the abbreviated names of
                         IEEE journals. (For use with IEEE work.)
                         
IEEEfull.bib           - String definitions for the full names of IEEE
                         journals. (Do not use for IEEE work.)


Carried on CTAN only, for non-IEEE related work:

IEEEtranSA.bst         - Like IEEEtranS.bst, but with alphanumeric citation
                         tags like alpha.bst. Not for normal IEEE use.

EEEtranN.bst          - Like IEEEtran.bst, but based on plainnat.bst and
                         is compatible with Patrick W. Daly's natbib
                         package. Not for normal IEEE use.

IEEEtranSN.bst         - Sorting version of IEEEtranN.bst. Not for normal
                         IEEE use

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran_bst_HOWTO.pdf, IEEEtran.bst, IEEEtranS.bst,
                   IEEEtranSA.bst, IEEEtranN.bst, IEEEtranSN.bst,
                   IEEEexample.bib, IEEEabrv.bib, IEEEfull.bib
                   
***************************************************************************


==> archive/content.tex <==
\begin{abstract}
Speech separation remains a particularly challenging area of speech processing in many scenarios. \Ac{DNN} based speech separation models can be separated into two classes depending on whether they make predictions using the entire sequence of input data or a selected window of context of the input data often referred to as the \ac{RF}.
This paper investigates firstly how much the fixed window size limits the performance of \ac{TCN} based speech separation models in far field scenarios and secondly where, if at all, the best place is in the network to introduce information from the full input audio sequence by inserting the output of a Transformer encoder layer at various stages in the network.
Evaluations are performed on numerous benchmarks to observe how the type of data effects where the optimal position of the global context layer is in the overall TCN.
\end{abstract}

\begin{IEEEkeywords}
speech separation, context modelling, convolutional neural networks,
\end{IEEEkeywords}
%

%%%%%%%%%%%%%%%%%%%%%%
% Introduction
%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:intro}
% Speech separation in general
Speech separation models are used in a number of downstream speech processing applications from meeting transcription and speaker recognition to hearing aids \cite{FFASRHaebUmbach,Raj2021IntegrationOS,ssha}. In many of these applications the speakers are at a far-field distance from the microphone which introduces additional challenges to the speech separation task due to interference from noise and reverberation in the signal \cite{chime5, IWAENCbestpaper}. 

% Fixed window vs. variable window models
\Ac{DNN} models have led to significant improvements in speech separation models on anechoic data but their is a significant performance gap when these models are used for more distorted speech data \cite{WHAMR, sepformer,QDPN} and so this in this paper the focus is on the more challenging far-field scenario. In this work it is proposed to consider the types of \ac{DNN} speech separation models in two separate classes, namely \ac{RF} models and \ac{FC} models. \Ac{RF} models are described in this paper as models which only process a select amount of temporal context for each output frame within the overall model's \ac{RF}. Typically these models are fully convolutional by design. \Ac{FC} models are described as models which observe for the full input sequence information in order to produce each output frame. The best performing \ac{FC} models typically contain many carefully structured recurrent or transformer layers then encode the information from the entire sequence \cite{sepformer,dprnn}. Because of this \ac{FC} models typically carry significantly more computational complexity \cite{sudormrf}.

% Data
A number of corpora have been proposed for speech separation model training, evaluation or both. WSJ0-2Mix was proposed in \cite{Isik} for monaural speech separation tasks. The speech is anechoic and contains a negligible level of noise making it a simple but unrealistic tasks for speech separation models in most applications. Impressive results have been achieved \cite{QPDN, sepformer} on WSJ0-2Mix and WSJ0-3Mix but the performance often significantly degrades when reverberation and noise are introduced into the task. The WHAMR dataset was proposed as a more challenging dataset. WHAMR is created in a similar wayt o WSJ0-2Mix but includes noise from urban environments and the speech is reverberated using \acp{RIR} from the pyroomacoustics toolkit \cite{pyroomacoustics}. WSJCAM-Mix is an attempt to move further away from the simulated approach using what the authors refer to as a "semi-simulated" method to create data. Single speaker utterances are recorded in a realistic environment using both a far field microphone to provide the input signal and headset microphone to provide a target signal. The far field data is then artificially overlapped. The only simulated parts of the process are the speech mixing and the extension of the noise signal in the short of the utterance which is often a negligible as more commonly when training and evaluating for the lone speech separation task, the longer utterance is truncated as opposed to extending the shorter utterance.

% In this work modelling
Using the a novel \ac{TCN} speech separation is introduced which incorporates a \ac{GRU} based network block which is configured to provide provide full sequence context at varying points in the \ac{TCN}. The motivation for this work is that while \acp{TCN} are one of the more parameter and computationally efficient models proposed \cite{sudormrf}, an obvious limitation of \acp{TCN} is the limited \ac{RF} for observing input data. As such it is investigated where, if at all, in the network is best to introduce this information by replacing each temporal convolutional block with the proposed \ac{GRU} block. The goal of this research is to maximise performance while maintaining a low computational cost by only introducing this information at one point in the network. it is thought that with the knowledge of where it best to introduce this information, subsequent work can focus on optimising the computational performance of the proposed structure as all \ac{RNN} layers, of which the \ac{GRU} layer is one, are known to have significant time-complexity \cite{Vaswani}.

% Paper structure
\section{Signal Model}
We define a noisy reverberant speech separation problem as trying to find some estimate of speech signal $s_c$ for C speech signals, i.e. $c\in\{1,\ldots,C\}$, denoted $\hat{s}_c$ from the discrete time domain mixture signal of length $L_x$ denoted
\begin{equation}
    x[i] = \sum_{c=1}^{C} s_c\ast h_c [i] + \nu [i]
\end{equation}
where $\ast$ denotes the convolution operator, $h_c$ is a \ac{RIR} corresponding to speaker $c$ and $\nu$ denotes an additive background noise source.

%%%%%%%%%%%%%%%%%%%%%%
% Separation network
%%%%%%%%%%%%%%%%%%%%%%
\section{Full Context Temporal Convolutional Speech Separation Networks}
In this section a model is introduced which replaces convolutional blocks in the \ac{TCN} with \ac{GRU} blocks. The motivation for this is that by using \ac{GRU} layers it is possible to encode information from the full input sequence. Furthermore when bidirectional \ac{GRU} layers are used, each output frame has access to the full sequence information as opposed to just what information has come before it.

The \ac{TCN} structure used is the same that described in \cite{atttasnet} which is a variation on the Conv-TasNet model \cite{convtasnet} that neglects the skip connection layers in the original. The network is composed of a series of convolutional blocks which contain a \ac{P-Conv} layer, PReLU activation, \ac{gLN} and \ac{DS-Conv} layer with a residual connection going around the entire block. The \ac{DS-Conv} layer is composed of a \ac{D-Conv} layer, \ac{PReLU} activation, \ac{gLN} and \ac{P-Conv}. For a more in depth explanation of this structure see \cite{atttasnet,convtasnet}. The convolutional blocks are stacked in a stack of $X$ blocks with increasing dilation factors in powers of two $f\in\{2^0,2^1,\ldots,2^{X-1}\}$. This stack is then repeated $R$ time with the dilation factor reset to $f=1$ at the start of each stack.

In the proposed network, one convolutional block of the entire \ac{TCN} is replaced by one of the GRU blocks described in Fig.~\ref{fig:grublock}. The motivation here is to asses the most appropriate place to introduce information from the entire sequence.
\begin{figure}
    \centering
    \input{GRUTemporalBlocks.pdf_tex}
    \caption{(a) Convolutional TCN block. (b) Proposed GRU block.}
    \label{fig:grublock}
\end{figure}

\section{WSJCAM-2Mix}
The WSJCAM-2Mix corpus of far-field speech mixtures is proposed in this work as a solution to training speech separation models on more realistic datasets. The WSJCAM0 dataset is selected as the source of single speaker far field data as it contains a reasonably simple scenario with only two microphones, one headset and one far-field desk microphone. The WSJCAM-2Mix corpus generation scripts are located at \footnote{WSJCAM-2Mix scripts: \url{https://github.com/jwr1995/WSJCAM-2Mix}}. The training data is drawn from the \textit{si\_tr} subset. Cross validation data is drawn from the \textit{si\_dt} subset and evaluation data is drawn from the \textit{si\_et\_1} subset.

% Peprocessing
%% Removal of short utterances
In first stage of preprocessing data, all utterances with 4 words or fewer are removed. This is due to some audio clips containing no speech and other clips only containing a few milliseconds of audio. In all this amounted to removing 225 utterances leaving 9182 utterances for training data, 1701 for validation data and 1222 for test data.

%% Cross correlation alignment
Empirically it was found the variation in delay between the headset audio and desk audio caused major issue when trying to train speech separation network. So the audio is aligned using a cross-correlation method, i.e. the far-field signal $s_{\mathrm{far},c}[i]$ is shifted forward in time by 
\begin{equation}
    \tau={\argmax(s_{\mathrm{far},c}\star s_{\mathrm{dir},c})}-{L_x}
\end{equation}
samples where $\star$ denotes the cross-correlation operator.

Two speaker mixtures are created by overlapping the speech segments at varying \acp{SSR} between 0 and 5~dB.
\begin{align*}
    \mathrm{SDR}_{\mathrm{RMS}}\left(s_{\mathrm{far},c} ,s_{\mathrm{dir},c}\right) &= \frac{1}{\frac{s_{\mathrm{far},c}}{s_{\mathrm{dir},c}}-1} \\
    \mathrm{SDR}_\mathrm{dB}\left(s_{\mathrm{far},c} ,s_{\mathrm{dir},c}\right) &= 20\log_{10}\left(\frac{1}{\frac{s_{\mathrm{far},c}}{s_{\mathrm{dir},c}}-1}\right) \text{dB}
\end{align*}

% Other metadata
Other metadata is also extracted from the WSJCAM0 corpus to aid researchers in analysing models in terms of gender, dialect and age. These are included in the mixture configuration \textit{.csv} files found in the \textit{data} folder.

\section{Experimental Setup}

\section{Results}
\begin{figure}
    \centering
    \includesvg[width=\columnwidth]{wsjcam-2mix.svg}
    \caption{\Ac{SISDR} (dB) results against position of \ac{GRU} block in \ac{TCN}. Colour indicates blocks of identical dilation factors in the none recurrent \ac{TCN}.}
    \label{fig:my_label}
\end{figure}

\bibliographystyle{IEEEbib}
\bibliography{refs}

\end{document}


==> q_table.tex <==
\begin{table}[!h]
\centering
\caption{Quartiles of mixture signal lengths in the WHAMR \textit{tt} evaluation set.}
\label{tab:quartiles}
\begin{tabular}{|c|c|c|}
\hline
\textbf{Quartile} & \textbf{Lower Bound (s)} & \textbf{Upper Bound (s)} \\ \hline
Q1                & 1.62                     & 4.67                     \\
Q2                & 4.67                     & 5.522                    \\
Q3                & 5.522                    & 6.724                    \\
Q4                & 6.724                    & 13.87                    \\ \hline
\end{tabular}
\end{table}
